Feedforward in Generative AI: Opportunities for a Design Space

Generative AI (GenAI) models have become more capable than ever at augmenting productivity and cognition across diverse contexts. However, a fundamental challenge remains as users struggle to anticipate what AI will generate. As a result, they must engage in excessive turn-taking with the AI's feedback to clarify their intent, leading to significant cognitive load and time investment. Our goal is to advance the perspective that in order for users to seamlessly leverage the full potential of GenAI systems across various contexts, we must design GenAI systems that not only provide informative feedback but also informative feedforward -- designs that tell users what AI will generate before the user submits their prompt. To spark discussion on feedforward in GenAI, we designed diverse instantiations of feedforward across four GenAI applications: conversational UIs, document editors, malleable interfaces, and automation agents, and discussed how these designs can contribute to a more rigorous investigation of a design space and a set of guidelines for feedforward in all GenAI systems.

==> sections/99_conclusion.tex <==
\section{Conclusion}
\label{section:conclusion}



==> versions/prev/2_critique.tex <==
\section{Critique of GenAI Interfaces Through the Lens of Feedforward}
% \section{Critique Through the Lens of Feedforward}
\label{section:critique}

In order to understand a wider range of needs and use cases for feedforward in GenAI, we must reflect and critique past and current GenAI systems and explore how we may improve on them.
We use a critical lens \cite{MBL2021generativetheoriesinteraction} with our perspective that GenAI systems need sufficient feedforward to assess and critique three GenAI systems the first author contributed to designing and implementing: Sensecape \cite{sensecape}, Luminate \cite{luminate}, and Malleable Overview-Detail Interfaces \cite{malleableODI}.

% In order to understand a wider range of needs and use cases for feedforward in GenAI, we must reflect and critique past and current systems. 
% This critical lens is to help us concretely understand

\paragraph{Malleable Overview-Detail Interfaces}


\paragraph{Luminate}
% 


\paragraph{Sensecape}
% Describe what the system is and what it's for. Then describe key features.
% Then, go into several of those features and say, however, the user may not know X or Y.
% Leads them to wonder, what will this be?


==> versions/prev/3_feedforward_prompting.tex <==
\section{Feedforward Prompting}
\label{section:feedforward_prompting}


% Features and various applications of this prompting method

% - Textual Outline Preview (Update: this should be a more direct representation, not just literally an outline component)
% - Preview of multiple possible interpretations (instead of asking, did you mean Apple the fruit or company, it just gives you two possible outputs, and lets you choose by either clicking which one, or keep typing to add more context to your prompt)
% - Outline is Directly Expandable/Modifiable -- slowly can become the response itself
% - Directly revies the previous output (you can also choose to ignore this if you'd like)
% - Select + Feedforward = 

% Types of Feedforward
% - Outline (Anticipated content and structure it will generate)
% - Where you will reivse content (hint by creating a gap/shade at a location)
% - How much content you will revise (hint by visually expanding something some length)
% - What the tone may sound like (hint with concrete phrases)
% - What kinds of representations you might want (hint at showing a bullet point list, but you switch to table)
% - 

% Feedforward + Chain of Thought
% Chain of Thought begins as the user types. These "chains" then can be further expanded by the user, where the user can explore each step of the chain that the LLM anticipates will be the change...
% The end-user is then able to adjust the stages

% The core idea about feedforward prompting is an interaction paradigm that prompts you to add more context to your prompt. It's this very rapid back and forth, incremental understanding of one another to reach this ideal prompt that has a good idea of what you might want to get....




% Maybe this workshop paper will explore three case studies, maybe:
% 1) Conversational Interface
% 2) Writing System
% 3) Generative UI


% Maybe with Graphic Art, you have heavier loads of generation, like selecting and autofill. and the feedforward is showing the actual scope it might change as well...
% Or maybe what will be replaced, what won't, what might shift -- these results also affords users to make more granular changes, since they have the control to do so now.
% I think I can still explore this kind of pattern on a writing interface as well. First making broad strokes and changes, but feedforward provides hints at what text will be revised, and basically prompts users to make more granular changes.

% Maybe the exploration is really the design space of understanding the representations necessary for diverse kinds of LLM feedforward info.

% Various applications: Generative and Malleable UI, Graphics/Design, Direct Text Editing

==> versions/prev/4_study.tex <==
\section{User Study}
\label{section:user_study}

\subsection{Procedure}

The first author used FeedforwardChat for four weeks.

\subsection{Results and Reflections}





==> versions/prev/5_discussion.tex <==
\section{Discussion}
\label{section:discussion}


\subsection{Practical Implications for Feedforward Prompting}

Of course, prompting an LLM continuously before the user submits their prompt is significantly most costly over submitting the prompt just once, once the user is ready.

% But user might not be ready, and the cognitive costs is pretty heavy.


\subsection{}


% Does this work well with Chain of Thought actually?
% Maybe this approach will actually incentivize self-prompt-chaining???
% What are the implications of this?


% A benefit of this is certainly more transparency in the LLM
% LLM is so flexible that adding this kind of structure is still okay for the LLM



% What's more costly, entering a prompt, then responding and saying, no i want this, or typing a prompt, and tuning the prompt/expected output to reduce message exchanges?

% Learning to become a better prompter. One is by trial and error experience. Perhaps another is through this feedforward that tells you what you might be able to anticipate.

==> versions/prev/9999_background.tex <==
\section{Background}
\label{section:background}

\subsection{Bridging the Gulf of Envisioning in LLM Interaction}
% Bridging the gulf of envisioning
% Why johnny can't prompt
% Grounded abstraction matching
% ...

% What are various proposed solutions in this.. gap?
% List the possible things in Hari's paper
% Grounded abstraction matching
% Piryan's IUI(?) paper
% ...
% Our approach: We take the perspective that the challenges that users have with anticipating what the LLM will provide as a response is an interface design limitation. Our core focus is to explore how we can help users expect what the LLM will respond by exploring interface solutions.


% There's also a huge world of literature surroudning AI agents + AI planning. This is sort of... anticipating what the AI is going to do. 


\subsection{Supporting Feedforward in Interactive Systems}
% Feedforward is a thing that describes an interface solution that helps users what they can expect from an interaction.
% For instance, ...
% This is often complementary to "feedback" where feedback is about telling users what happened after they performed an action, whereas "feedforward" is about tellings users what will, might, and can happen before they perform the action.
% Octopocus


\subsection{Prompting Techniques}



